Student Usage of Q&A Forums: Signs of Discomfort?

Q&A forums are widely used in large classes to provide scalable support. In addition to offering students a space to ask questions, these forums aim to create a community and promote engagement. Prior literature suggests that the way students participate in Q&A forums varies and that most students do not actively post questions or engage in discussions. Students may display different participation behaviours depending on their comfort levels in the class. This paper investigates students' use of a Q&A forum in a CS1 course. We also analyze student opinions about the forum to explain the observed behaviour, focusing on students' lack of visible participation (lurking, anonymity, private posting). We analyzed forum data collected in a CS1 course across two consecutive years and invited students to complete a survey about perspectives on their forum usage. Despite a small cohort of highly engaged students, we confirmed that most students do not actively read or post on the forum. We discuss students' reasons for the low level of engagement and barriers to participating visibly. Common reasons include fearing a lack of knowledge and repercussions from being visible to the student community.

==> 01intro-old.tex <==
\section{Introduction}
\label{intro}
Due to increased interest and growing class sizes in computer science, online Q\&A forums such as Piazza have become increasingly important~\cite{barker2003online,thinnyun2021gender,joynerDoubleEdged}. Q\&A forums offer a scalable way for students to seek help from course instructors and teaching assistants while also providing space to discuss with other students. However, previous work in computing courses suggests that participation improves course performance or that only stronger students participate in Q\&A forums~\cite{dezausing, nandi2011active}.

Literature suggests that most students do not participate actively in Q\&A forums~\cite{nandi2011active}. While it is unclear whether there are negative consequences for not contributing visibly~\cite{edelmann2013reviewing}, general board engagement can encourage reflection on course material and has been linked to better course performance~\cite{ryle2007reflections, anderson2000computer}.
Reasons for not participating in Q\&A forums include low academic confidence~\cite{mazuro2011online, tafliovich2013student}, being in a minority group (gender or ethnic), and large class sizes~\cite{ruthotto2020lurking}. Since these forums are intended to support all students, it is important to consider what factors affect students' comfort with seeking help and if their lack of participation is influenced by factors instructors can fix.

Prior work also suggests that students use anonymity  differently~\cite{thinnyun2021gender, joynerDoubleEdged, brigham2021gender}, implying that there are different levels of comfort among students in a class. However, we did not find work that attempts to merge participation, viewing, usage of anonymity, private posts, and general student expectations from a Q\&A environment for a holistic view of such environments in a computing course.

In this paper, we investigate Piazza usage data from two offerings of a CS1 course. We look at patterns in student viewing and posting activities. We also consider gender differences in the usage of anonymity and report student perspectives on anonymity and Q\&A forums in general to identify reasons why students choose to be anonymous to peers and to illustrate a connection to status theory. Specifically:

\begin{description}
    \item[\textbf{RQ1}:] How do students typically use (post, reply, read) a Q\&A forum in a CS1 course?
    \item[\textbf{RQ2}:] How does anonymous usage of the board connect with engagement and demographic factors?
\end{description}

In the next section, we describe theory related to participation in online communities and prior work on related behaviour.
